HyperFields: Towards Zero-Shot Generation of NeRFs from Text

We introduce HyperFields, a method for generating text-conditioned Neural Radiance Fields (NeRFs) with a single forward pass and (optionally) some fine-tuning. Key to our approach are: (i) a dynamic hypernetwork, which learns a smooth mapping from text token embeddings to the space of NeRFs; (ii) NeRF distillation training, which distills scenes encoded in individual NeRFs into one dynamic hypernetwork. These techniques enable a single network to fit over a hundred unique scenes. We further demonstrate that HyperFields learns a more general map between text and NeRFs, and consequently is capable of predicting novel in-distribution and out-of-distribution scenes -- either zero-shot or with a few finetuning steps. Finetuning HyperFields benefits from accelerated convergence thanks to the learned general map, and is capable of synthesizing novel scenes 5 to 10 times faster than existing neural optimization-based methods. Our ablation experiments show that both the dynamic architecture and NeRF distillation are critical to the expressivity of HyperFields.

==> author.tex <==
\author{%
\resizebox{\textwidth}{!}{%
Sudarshan Babu$^{*\dagger}$%
~
Richard Liu$^{*\ddagger}$%
~
Avery Zhou$^{*\dagger \ddagger}$%
~
Michael Maire$^{\ddagger}$%
~
Greg Shakhnarovich$^{\dagger}$%
~
Rana Hanocka$^{\ddagger}$%
}\\
\resizebox{0.95\textwidth}{!}{
\begin{minipage}[t]{\linewidth}
\vspace{-7pt}
\begin{center}
\hfill
\begin{minipage}[t]{0.50\linewidth}
\centering
$^{\dagger}$\textit{Toyota Technological Institute at Chicago}\\
\scriptsize{\texttt{\{sudarshan,greg\}@ttic.edu}} 
\end{minipage}%
\hfill
\begin{minipage}[t]{0.49\linewidth}
\centering
$^{\ddagger}$\textit{University of Chicago}\\
\scriptsize{\texttt{\{guanzhi,averyzhou,mmaire,ranahanocka\}@uchicago.edu}}
\end{minipage}%
\hfill
\end{center}%
\vspace{5pt}
\begin{center}
\hfill
\begin{minipage}[t]{0.99\linewidth}
\centering
$^*$ Equal contribution
\end{minipage}%
\hfill
\end{center}
\end{minipage}%
}%
}

==> iclr_stuff/iclr2024_conference.tex <==
\input{header}

% Optional math commands from https://github.com/goodfeli/dlbook_notation.
\input{math_commands.tex}

%\usepackage{hyperref}
%\usepackage{url}

\input{macros}

\title{HyperFields: Towards Zero-Shot Generation of NeRFs from Text}

% Authors must not appear in the submitted version. They should be hidden
% as long as the \iclrfinalcopy macro remains commented out below.
% Non-anonymous submissions will be rejected without review.



% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to \LaTeX{} to determine where to break
% the lines. Using \AND forces a linebreak at that point. So, if \LaTeX{}
% puts 3 of 4 authors names on the first line, and the last on the second
% line, try using \AND instead of \And before the third author name.

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

%\iclrfinalcopy % Uncomment for camera-ready version, but NOT for submission.
\begin{document}
%\input{author}

\maketitle

\input{images/teaser.tex}
\input{abstract}
\input{introduction}
\input{related_work}
\input{method}
\input{results}
\input{conclusion}

\bibliography{iclr2024_conference}
\bibliographystyle{iclr2024_conference}
\pagebreak
\input{supp_paper}
\end{document}


==> old.tex <==
\input{header}

% Optional math commands from https://github.com/goodfeli/dlbook_notation.
\input{math_commands.tex}

%\usepackage{hyperref}
%\usepackage{url}

\input{macros}

\title{HyperFields: Towards Zero-Shot Generation of NeRFs from Text}

% Authors must not appear in the submitted version. They should be hidden
% as long as the \iclrfinalcopy macro remains commented out below.
% Non-anonymous submissions will be rejected without review.



% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to \LaTeX{} to determine where to break
% the lines. Using \AND forces a linebreak at that point. So, if \LaTeX{}
% puts 3 of 4 authors names on the first line, and the last on the second
% line, try using \AND instead of \And before the third author name.

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

%\iclrfinalcopy % Uncomment for camera-ready version, but NOT for submission.
\begin{document}
%\input{author}

\maketitle

%\input{images/teaser.tex}
\input{abstract}
%\input{introduction}
%\input{related_work}
%\input{method}
%\input{results}
%\input{conclusion}

%\bibliography{iclr2024_conference}
%\bibliographystyle{iclr2024_conference}
\pagebreak
%\input{supp_paper}
\end{document}


==> trash.tex <==


%\begin{cooment}
%\begin{figure*}
%    \centering
%    \includegraphics[width=1\textwidth]{images/compare_convergence_clear.png}
%    \caption{\textbf{Comparing number of epochs to convergence:} On an average our method converges at least 5 times faster than both the fine tuned (F) and trained from scratch (S) baselines. As soon as a scene reasonably describes the given prompt we consider the model to have converged. In a few instances the baselines never generates a scene close to the text prompt, in which case we stop the run at 150 epochs.}
%    \label{fig:oodconv}
%\end{figure*}
%\end{comment}
%\begin{comment}
%\section{Convergence to Out of Distribution Geometry}
%\label{sec:ood}
%\begin{figure}
        %\centering
        %\includegraphics[width=\columnwidth]{images/ood_generalization.png}
        %\caption{\textbf{Out of Distribution Generalization.} We train a single \ourmethod{} model and compare Stable DreamFusion. ``Stable DreamFusion (F)" indicates finetuning from an initialized DreamFusion model. ``Stable DreamFusion (S)" indicates the DreamFusion model trained from scratch. Zero-shot results and initializations are shown in the upper left of ``Ours" and ``Stable DreamFusion (F)", respectively. Above each column indicates the number of epochs each method is trained for. }
        \label{fig:ood_sup}
%\end{figure}

%Figure 8 in the main paper shows a few examples (gold blender, plaid skateboard) of our model converging significantly faster than the baselines to a shape the model has not seen during training using the same optimization signal (Score Distillation Sampling). In this section we extend those results to more objects. \cref{fig:ood} shows that our model generates desirable shape and texture at very few epochs when compared to the fine-tuned baseline and the baseline trained from scratch. The fine tuned baselines are initialized to a NeRF that produces the same object predicted by our model zero shot. The initialization is illustrated in top left corner of the fine tuned baseline results, while similarly the zero shot results are on the top left corner of our model's results (Figure 3). 

%In \cref{fig:oodconv} we compare the time to converge to a scene that reasonably represents the given prompt. From \cref{fig:oodconv}, we see that our model on an average converges 5 times faster than the baselines. From \cref{fig:oodvisual} we see that our model generates better quality scenes than the baselines. \textbf{Gold Blender:} the geometry for blender for both baselines is more similar to a cup, whereas ours has the shape of blender. \textbf{Plaid Skateboard:} The fine tuned model has the board mounted on box like shape, and the trained from scratch model is not as plaid-like, while our model generates a skateboard with a strong plaid texture to it. \textbf{Glacier Knife:} While the basic knife structure is present, the fine tuned model ignores the glacier texture. \textbf{Yarn Shoes:} All 3 models  model converge to reasonable shape and texture, although the shoes are kept mounted in the fine tuned model. \textbf{Plaid Lamp Post:} The trained from scratch model ignores the plaid attribute completely, and the synthesized lamppost is very small. The finetuned baseline simply creates a light from inside the toaster intialization. \textbf{Victorian Teapot:} The basic geometry seems to be present in all 3 models, however the handle is better placed in ours than in the baselines. \textbf{Strawberry with Tiger Stripes:} The shape of the fine tuned model looks more like a pineapple than a realistic strawberry, and the scratch baseline model does not have visible tiger stripes. \textbf{Yarn Skateboard:} With the yarn skateboard our geometry is more similar to a skateboard, while the fine tuned model does not move much beyond the bowl initialization, and the scratch baseline generates a plausible skateboard (albeit with some janused wheels) without any visible yarn texture.



%\clearpage

%\end{comment}






%\begin{figure}
%    \centering
%    \includegraphics[width=0.8\columnwidth]{images/speedup.png}
%    \caption{\textbf{5-10x Convergence.} \ourmethod{} (Ours) enables several times faster convergence of novel scenes from scratch compared to the baseline (Stable DreamFusion (F)) initialized in the same way as Fig.~\ref{fig:stylebaseline} \rl{TODO: put from scratch in here. also numbers above the bars! Also, report the stuck local minima!}}. 
%    \label{fig:speedup}
%\end{figure}





%{\small
%\bibliographystyle{ieee_fullname}
%\bibliography{supp_bib}
%}
%\end{document}  


%\end{appendices}
